Need Help? Designing Proactive AI Assistants for Programming

While current chat-based AI assistants primarily operate reactively, responding only when prompted by users, there is significant potential for these systems to proactively assist in tasks without explicit invocation, enabling a mixed-initiative interaction. This work explores the design and implementation of proactive AI assistants powered by large language models. We first outline the key design considerations for building effective proactive assistants. As a case study, we propose a proactive chat-based programming assistant that automatically provides suggestions and facilitates their integration into the programmer's code. The programming context provides a shared workspace enabling the assistant to offer more relevant suggestions. We conducted a randomized experimental study examining the impact of various design elements of the proactive assistant on programmer productivity and user experience. Our findings reveal significant benefits of incorporating proactive chat assistants into coding environments and uncover important nuances that influence their usage and effectiveness.

==> files/usability_study.tex <==
\section{Usability Study} \label{sec:usability_study}

\vccomment{contrast with motivation for controlled study, follow-up...}

\textbf{Over time:} We focus on this less in this work... \vccomment{omit or revisit?}
\begin{itemize}
    \item \textit{DP3.1: Remember recent interactions.}
    \item \textit{DP3.2: Learn from user behavior.}
    \item \textit{DP3.3: Provide global controls.}
    \item \textit{DP3.4: Integration with other services.}
\end{itemize}

\textbf{RQ5:} How does the proactive assistant integrate with existing coding tools (e.g., Copilot)?

\paragraph{Perceived integration with existing workflows} This is only relevant to the usability study. This is measured by... \vccomment{check if any prior study did this.}

\subsection{Study details}

\vccomment{recall what the goals of the usability study is}. what experimental conditions are relevant.. \vccomment{mention the amount of time, do the study asynchronously}

\subsection{Results}

